Scalar curvature rigidity of domains in a 3-dimensional warped product

A warped product with a spherical factor and a logarithmically concave warping function satisfies a scalar curvature rigidity of the Llarull type. We develop a scalar curvature rigidity of the Llarull type for a general class of domains in a three dimensional spherical warped product. In the presence of rotational symmetry, we identify this class of domains as those satisfying a boundary condition analogous to the logarithmic concavity of the warping function.

==> spherical.tex <==
\label{sec:spherical_part}


This part is a slightly extension of the argument in Section 5 in our previous paper \cite{chai-scalar-2023-arxiv}.
So we only sketch the key steps here and refer to the previous paper for more details.

Suppose $M$ is given by
\[
	M=\left\{ (t^2, r, \theta): t\in [0, \varepsilon), r \in [0, \phi(t)), \theta \in \mathbb{S}^1 \right\},
\]
near $p^+=O$ for some smooth function $\phi(0)=0$.
Note that we need to assume $\psi(0)\neq 0$, otherwise the manifold $M$ will have a cusp at point $O=(0,0,0)$.
%If $k=1$, then $M$ is a manifold with a conical singularity at $O$.
%The boundary of $M$ near $O$ is given by
%\[
	%\partial M=\left\{ (t^k,\phi(t),\theta): t \in [0,\varepsilon),\theta \in \mathbb{S}^1 \right\}.
%\]

%We define the surface
%\[
	%\Sigma_t= \left\{ x=t^k \right\}\cap M
%\]
%and
%\[
	%\Sigma_{t,u}=\left\{ (t^k+u(\hat{x}), \phi((t^k+u(\hat{x}))^{\frac{1}{k}})\hat{x}):\hat{x} \in D \right\}.
%\]

%In particular, we can find
%\begin{align*}
	%\frac{H_{t,t^{k+1}u}-\overline{h}_{t,t^{k+1}u}}{t^{k-1}}={} & \frac{t^2}{\phi^2(t)}\Delta_t u+\frac{H_t-\overline{h}_t}{t^{k-1}}+O(t),\\
	%\frac{\cos \gamma_{t,t^{k+1}u}-\cos \overline{\gamma}_{t,t^{k+1}u}}{t^{2k-1}} 
	%={}& 
	%\frac{\sin \gamma_t}{\phi(t)t^{k-2}}\frac{\partial u}{\partial \nu_t}+(A_{\partial M}(\eta_t,\eta_t)-\cos \gamma_t A(\nu_t,\nu_t)\\
	%{}& -\overline{A}_{\partial M}(\overline{\eta}_t,\overline{\eta}_t))\frac{u}{t^{k-2}}+\frac{\cos \gamma_t-\cos \overline{\gamma}_t}{t^{2k-1}}+O(t).
%\end{align*}

%There are two subcases we need to consider.
%The first one is $g=\overline{g}$ at $O$.


%The second case is that $g> \overline{g}$ at $O$.

To better illustrate the situation, we use the stereographic projection to describe the metric on sphere.
So the manifold $M$ can be written as
\[
	M=\left\{ (t^2,x,y):t \in [0,\varepsilon), x^2+y^2\le \tan^2(\phi(t)) \right\},
\]
and the background metric $\overline{g}$ is given by
\[
	\overline{g}=dt^2+\frac{\psi^2(t)(dx_1^2+dx_2^2)}{(1+|x|^2)^2}=dt^2+\psi^2(0)(dx_1^2+dx_2^2)+O(t)+O(|x|^2),
\]
where $|x|=\sqrt{x_1^2+x_2^2}$.
For simplicity, we denote $\overline{g}_0=dt^2+\psi^2(0)(dx_1^2+dx_2^2)$ as the linearised part of $\overline{g}$ at $O$.
After a suitable rotation, we can write $g=g_0+th+O(t^2)$ for some constant metric $g_0$ defined as
\begin{equation}
	g_0=a_{33}dt^2+(a_{11}dx_1^2+a_{22}dx_2^2)+2a_{13}dx_1dt+2a_{23}dx_2dt,
	\label{eq:G0Def}
\end{equation}
where the matrix
\[
	\begin{bmatrix}
		a_{11} & 0 & a_{13}\\
		0 & a_{22} & a_{23} \\ 
		a_{13} & a_{23} & a_{33}
	\end{bmatrix}
\]
is positive definite and satisfies $a_{11},a_{22}\ge \psi^2(0)$, $a_{33}\ge 1$.
We assume $\partial M$ is given by
\[
	M=\left\{ (\zeta(|x|^2),x): |x|\le \varepsilon \right\}
\]
near $O$ for some smooth function $\zeta$ with $\zeta(0)=0$ and $\zeta'(0)>0$ and $\varepsilon>0$ small enough.
Indeed, $\zeta$ is defined as
\[
	\zeta(r^2)=(\phi^{-1}(\arctan(r)))^2.
\]
and we can check $\zeta$ is smooth with $\zeta(0)=0$, $\zeta'(0)>0$ by the property of $\phi$.



We write $a^{ij}$ as the inverse matrix of $a_{ij}$ and consider the function $G_{s,t}$ defined by
\[
	G_{s,t}(x_1,x_2)=\zeta'(0)x_1^2(\sqrt{a_{11}a^{33}}+s-1)+\zeta'(0)x_2^2(\sqrt{a_{22}a^{33}}+s-1),
\]
and the surface $\Sigma_{s,t}$ is defined by
\[
	\Sigma_{s,t}=\left\{ (G_{s,t}, x): G_{s,t}(x)\ge \zeta(|x|^2) \right\}.
\]
We use an ellipse $E_s$ to parameterize $\Sigma_{s,t}$ where $E_s\subset \mathbb{R}^2$ is given by
\[
	E_s:=\left\{ \hat{x} \in \mathbb{R}^2:(b_1+s)\hat{x}_1^2+(b_2+s)\hat{x}_2^2<1 \right\}.
\]
Then, the surface $\Sigma_{s,t}$ can be written as
\[
	\Sigma_{s,t}(\hat{x}):=(G_{s,t}(\Phi_{s,t}(\hat{x})),\Phi_{s,t}(\hat{x}))
\]
where $\Phi_{s,t}:E_s\rightarrow \mathbb{R}^2$ satisfies
\[
	\Phi_{s,t}(\hat{x})=\frac{t \hat{x}}{\sqrt{\zeta'(0)}}+O(t^3).
\]

We also use $\Sigma_t=\Sigma_{0,t}$ for short.
We have the following result by the argument in \cite{chai-scalar-2023-arxiv}.

\begin{proposition}
	\label{prop_angleAsy}
	Suppose the metric $g$ can be written as $g=g_0+th+O(t^2)$ where $g_0$ is the constant metric defined in \eqref{eq:G0Def} and $h$ is a bounded symmetric two-tensor.
	Then, we have
	\begin{align*}
		\cos \gamma_{s,t}(\hat{x})={}&\cos \bar{\gamma}_{s,t}(\hat{x})+2\zeta'(0)\hat{x}_\alpha^2 t^2\left( \frac{1}{\psi^2(0)}-\frac{(b_\alpha+s)^2}{a_{\alpha\alpha}a^{33}} \right)+A(\hat{x})t^3+L(h)t^3+O(t^4).
\end{align*}
	for any $\hat{x} \in E_s$.
	Here, $A(\hat{x})$ is a bounded term (not related to $t$ and $h$) which is also odd symmetric with respect to $\hat{x}$, $L(h)$ is a bounded term (not related to $t$) relying on $h$ linearly.
\end{proposition}
\begin{proof}
	[Sketch of the proof]
	We use the same argument for Proposition 5.16 in \cite{chai-scalar-2023-arxiv} to prove
\begin{align*}
	\cos \measuredangle _{g_0}(\Sigma_{s,t},\partial M)={}&1-\frac{2\zeta'(0)(b_\alpha+s)^2\hat{x}^2_\alpha}{a_{\alpha\alpha}a^{33}}t^2+A(\hat{x})t^3+O(t^4)\\
	\cos \overline{\gamma}_{s,t}(\hat{x})={}&1-\frac{2\zeta'(0)\hat{x}_\alpha^2t^2}{\psi^2(0)}+A(\hat{x})t^3+O(t^4).
\end{align*}
Together with the Corollary 5.5 in \cite{chai-scalar-2023-arxiv} (see the proof for Corollary 5.17 in \cite{chai-scalar-2023-arxiv}), we can establish the result.
\end{proof}

As a corollary, we can easily establish the following result for $\sin \gamma_t$ (cf. Corollary 5.18 in \cite{chai-scalar-2023-arxiv}):
\begin{equation}
\sin \gamma_{t}(\hat{x})=\sin \bar{\gamma}_t(\hat{x})+O(t^2)=2\sqrt{\zeta'(0)}\psi(0)|\hat{x}|t+O(t^2),\label{eq:corAngleSin}
\end{equation}



\begin{proposition}
	\label{prop_GreaterAngleG0}
	Suppose the conditions in Proposition \ref{prop_angleAsy} holds.
	Then, for any $s>0$, we can find $t_0>0$ (might rely on $s$) such that for any $t<t_0$, we have
	\begin{equation}
		\gamma_{s,t}(\hat{x})>\bar{\gamma}_{s,t}(\hat{x})
		\label{eq:corGreaterAngle}
	\end{equation}
	for any $\hat{x} \in \partial E_s$.
\end{proposition}

We need to analyze the asymptotic behavior of mean curvature.
We define the following mean curvatures:
\begin{align*}
	H_{s,t}^{g}(\hat{x}):={}&\text{Mean curvature of $\Sigma_{s,t}$ at $\Sigma_{s,t}(\hat{x})$ under metric $g$},\\
	H_{s,t,\partial M}^{g}(\hat{x}):={}& \text{Mean curvature of $\partial M$ at $(\varphi(|\Phi_{s,t}(\hat{x})|^2),\Phi_{s,t}(\hat{x}))$ under metric $g$}.
\end{align*}

\begin{proposition}
	\label{prop_meanAsy}
	Suppose the metric $g$ can be written as $g=g_0+t h+O(t^2)$ where $g_0$ is a constant metric defined in \eqref{eq:G0Def}, and $h$ is a bounded symmetric two-tensor. 
	Then, we have the following formula for the behavior of mean curvature
	\begin{equation}
		\label{eq:corMean}
		H^g_t(\hat{x})=H^g_{t,\partial M}(\hat{x})-H^{\overline{g}}_{t,\partial M}(\hat{x})+2\zeta'(0)\left( \frac{2}{\psi(0)}-\frac{1}{\sqrt{a_{11}}}-\frac{1}{\sqrt{a_{22}}} \right)+tL(\hat{x})+O(t^2),
	\end{equation}
	for any $\hat{x} \in E$.
	Here, we write $H^g_t=H^g_{0,t}$ and $H^g_{t,\partial M}=H^g_{0,t,\partial M}$ for short.
\end{proposition}

\begin{proof}
	[Sketch of the proof]
	We can establish the following mean curvature relations under metric $g_0$ (cf. Proposition 5.21 in \cite{chai-scalar-2023-arxiv}):
	\[
	H_t^{g_0}(\hat{x})-H_{t,\partial M}^{g_0}(\hat{x})=-\frac{2\zeta'(0)}{\sqrt{a_{11}}}-\frac{2\zeta'(0)}{\sqrt{a_{22}}}+tL(\hat{x}) +O(t^2),
	\]
	Note that by the proof for Corollary 5.9 in \cite{chai-scalar-2023-arxiv}, we can establish the following results:
\begin{align}
	H^{g}_{t,\partial M}(\hat{x})-H^{g_0}_{t,\partial M}(\hat{x}) ={} & H^{g}_{t}(\hat{x})-H^{g_0}_{t}(\hat{x})+tL(\hat{x})+O(t^2).
	%H^{\overline{g}}_{t,\partial M}-H^{\overline{g}_0}_{t,\partial M} ={} & H^{\overline{g}}_{t}-H^{\overline{g}_0}_{t}+tL(\hat{x})+O(t^2).
\end{align}
In particular, it implies
\begin{align}
	H^g_{t}(\hat{x})={}&H^{g_0}_{t}(\hat{x})-H^{g_0}_{t,\partial M}(\hat{x})+H^g_{t,\partial M}(\hat{x})+tL(\hat{x})+O(t^2)\\
	={}&H^g_{t,\partial M}(\hat{x})-2\zeta'(0)\left( \frac{1}{\sqrt{a_{11}}}+\frac{1}{\sqrt{a_{22}}} \right)+tL(\hat{x})+O(t^2)\\
	={}&H^g_{t,\partial M}(\hat{x})-H^{\overline{g}}_{t,\partial M}(\hat{x})+2\zeta'(0)\left( \frac{2}{\psi(0)}-\frac{1}{\sqrt{a_{11}}}-\frac{1}{\sqrt{a_{22}}} \right),
	%\label{eq:pfDiffMean}
\end{align}
where we have used the fact that $H^{\overline{g}_0}_{t,\partial M}(\hat{x})=\frac{4\zeta'(0)}{\psi(0)}+\overline{h}(0)+O(t^2)$ by a direct computation.
\end{proof}




%We have


%We also have
%\[
	%H_t^{\overline{g}_0}(\hat{x})-H_{t,\partial M}^{\overline{g}_0}(\hat{x})=-\frac{2\zeta'(0)}{\psi(0)}-\frac{2\zeta'(0)}{\psi(0)}+tL(\hat{x}) +O(t^2),
%\]

%Note that by the proof for Corollary 5.9 in ??, we can establish the following results:
%\begin{align}
	%H^{g}_{t,\partial M}(\hat{x})-H^{g_0}_{t,\partial M}(\hat{x}) ={} & H^{g}_{t}(\hat{x})-H^{g_0}_{t}(\hat{x})+tL(\hat{x})+O(t^2).
	%%H^{\overline{g}}_{t,\partial M}-H^{\overline{g}_0}_{t,\partial M} ={} & H^{\overline{g}}_{t}-H^{\overline{g}_0}_{t}+tL(\hat{x})+O(t^2).
%\end{align}

%In particular, it implies
%\begin{align}
	%H^g_{t}(\hat{x})={}&H^{g_0}_{t}(\hat{x})-H^{g_0}_{t,\partial M}(\hat{x})+H^g_{t,\partial M}(\hat{x})+tL(\hat{x})+O(t^2)\\
	%={}&H^g_{t,\partial M}(\hat{x})-2\zeta'(0)\left( \frac{1}{\sqrt{a_{11}}}+\frac{1}{\sqrt{a_{22}}} \right)+tL(\hat{x})+O(t^2)\\
	%={}&H^g_{t,\partial M}(\hat{x})-H^{\overline{g}}_{t,\partial M}(\hat{x})+2\zeta'(0)\left( \frac{2}{\psi(0)}-\frac{1}{\sqrt{a_{11}}}-\frac{1}{\sqrt{a_{22}}} \right),
	%\label{eq:pfDiffMean}
%\end{align}
%where we have used the fact that $H^{\overline{g}_0}_{t,\partial M}(\hat{x})=\frac{4\zeta'(0)}{\psi(0)}+\overline{h}(0)+O(t^2)$ by a direct computation.

Now, we consider
\[
	H_0:=\lim_{t\rightarrow 0} H_t^g(\hat{x}),
\]
which is well-defined by \eqref{eq:corMean} (the limit does not depend on the choice of $\hat{x}$.)

We have two subcases to consider.

If $H_0>\overline{h}(0)$, then we can use the continuation of $H_{s,t}^g$ with respect to $s$ and $t$, together with Proposition \ref{prop_GreaterAngleG0}, we can show the following results (cf. Proposition 5.10 in \cite{chai-scalar-2023-arxiv}).
\begin{proposition}
	\label{prop_GreaterMean}
	Suppose the metric $g$ can be written as $g=g_0+th+O(t^2)$ where $g_0$ is a constant metric defined in \eqref{eq:G0Def}, and $h$ is a bounded symmetric two-tensor.
	If $H_0>\overline{h}(0)$, we can choose some $s>0,t>0$ small such that $H_{s,t}^g(\hat{x})>\overline{h}(\Sigma_{s,t}(\hat{x}))$ for any $\hat{x} \in \partial E_s$ and $\gamma_{s,t}(\hat{x})>\overline{\gamma}_{s,t}(\hat{x})$ for each $\hat{x} \in \partial E_s$.
\end{proposition}

Now, we focus on the case $H_0=\overline{h}(0)$.
In particular, it implies $a_{11}=a_{22}=\psi(0)$ and $H^g_{\partial M}(O)=H^{\overline{g}}_{\partial M}(O)$.

Then, we need to construct a foliation near $O$.
We define the vector field $Y_t(\hat{x}):=\frac{\partial }{\partial t}\Sigma_t(\hat{x})$.
Given $u \in C^{1,\alpha}(\overline{E})\cap C^{2,\alpha}(E)$ where $E=E_0$, we can define the perturbation surface $\Sigma_{t,u}$ by
\[
	\Sigma_{t,u}:=
	\left\{ \Sigma_{t-\frac{u}{\left< Y_t(\hat{x}),N_t(\hat{x}) \right> }}(\hat{x}):\hat{x} \in E \right\}
\]
where $N_t(\hat{x})$ is the unit normal vector field of $\Sigma_t$.

Recall that
\[
	E=\left\{ \hat{x}:\psi(0)a^{33}|\hat{x}|^2<1 \right\}.
\]


Replace $u$ by $ut^3$ and assume $u=O(1)$, we have
\begin{align*}
	\frac{H_{t,t^3u}-\overline{h}_{t,t^3u}}{t}={} & -\Delta_t^E u+\frac{H_t-\overline{h}_t}{t}+O(t),\\
	\frac{\cos \gamma_{t,t^3u}-\cos \bar{\gamma}_{t,t^3u}}{t^3}={} & 
	-2\sqrt{\zeta'(0)}\psi(0)|\hat{x}| \frac{\partial u}{\partial \nu_t^E}+(A_{\partial M}(\eta_t,\eta_t)-\cos \gamma_t A(\nu_t,\nu_t)\\
&-\bar{A}_{\partial M}(\bar{\eta}_t,\bar{\eta}_t))u+
\frac{\cos \gamma_t-\cos \bar{\gamma}_t}{t^3}+O(t),
\end{align*}
where $\Delta_t^E$ denotes the Laplacian-Beltrami operator on $E$ under the metric $\frac{1}{t^2}\Sigma^*_t(g)$, and $\nu_t^E$ is the unit normal vector field of $\partial E$ under the metric $\frac{1}{t^2}\Sigma^*_t(g)$.
Here, we have used \eqref{eq:corAngleSin}.


By using the same argument for Proposition 5.27 in \cite{chai-scalar-2023-arxiv}, together with the asymptotic behavior of mean curvature and mean curvature, for each $t \in (0,\varepsilon)$ for $t$ small enough, we can find $u_t(\cdot)=u(\cdot,t)$ such that the mean curvature $H_{t,t^3u_t}$ is $\overline{h}_{t,t^3u}+t\lambda(t)$ where $\lambda(t)$ is a function only depends on $t$, the contact angle $\gamma_{t,t^3u_t}=\overline{\gamma}_{t,t^3u_t}$, and $u$ satisfies the following result
\[
	\lim_{t\rightarrow 0} (u(\hat{x},t)+u(-\hat{x},t))=0
\]
for any $\hat{x} \in E$.
A finer analyze of $\lambda_t$ will give us $\lambda_t>0$ for $t$ sufficiently small (cf. Proposition 5.28 in \cite{chai-scalar-2023-arxiv}), which leads to the following result.
\begin{proposition}
	\label{prop_meanConvexSphere}
	We can construct a surface $\Sigma$ near $O$ such that the mean curvature of $\Sigma$ is not less than $\overline{h}$ and it has prescribed contact angle $\overline{\gamma}$ with $\partial M$.
\end{proposition}

\begin{proof}
	[Proof of main theorem for spherical case]
	If $p^+$ (respectively, $p^-$) is a spherical point and $\psi(p^+)$ (respectively, $\psi(p^-)$) is not zero, then we can use Proposition \ref{prop_GreaterMean} or Proposition \ref{prop_meanConvexSphere} depending on the value of $H_0$ to construct a barrier surface $\Sigma$ with mean curvature not less than $\overline{h}$ and prescribed contact angle $\overline{\gamma}$ with $\partial M$.
	Then, we can use Theorem \ref{simple} to extend the rigidity to all of $M$.
\end{proof}



\

\


